Long-duration transient, gravitational-wave search pipeline

As the sensitivity and observing time of gravitational-wave detectors increase, a more diverse range of signals is expected to be observed from a variety of sources. Especially, long-lived gravitational-wave transients have received interest in the last decade. Because most of long-duration signals are poorly modeled, detection must rely on generic search algorithms, which make few or no assumption on the nature of the signal. However, the computational cost of those searches remains a limiting factor, which leads to sub-optimal sensitivity. Several detection algorithms have been developed to cope with this issue. In this paper, we present a new data analysis pipeline to search for un-modeled long-lived transient gravitational-wave signals with duration between 10 and 1000 s, based on an excess cross-power statistic in a network of detectors. The pipeline implements several new features that are intended to reduce computational cost and increase detection sensitivity for a wide range of signal morphologies. The method is generalized to a network of an arbitrary number of detectors and aims to provide a stable interface for further improvements. Comparisons with a previous implementation of a similar method on simulated and real gravitational-wave data show an overall increase in detection efficiency depending on the signal morphology, and a computing time reduced by at least a factor 10.

==> referee_answers2.tex <==
We thank the referee for their report and address their last comments below. Changes in the paper are highlighted in blue.

 L42: citations 10 and 11 are good overviews of CWs, but 12 and 13 are
two seemingly arbitrary search method references out of a large field
and there is no apparent reason for picking these two.

A: we have removed citations 12 and 13.

L255: the notation for pixel resolution is still confusing: Delta t
will generally be understood as having units of seconds already, so
explicitly multiplying by "s" and "Hz" would have the effect of
squaring the units here. They would still cancel out, but their
inclusion is confusing. Alternatively, this could be expressed in
words.

A: we have removed the units as they generate confusion.

L480 (Sec. II.B): the answer given by the authors about what
"coincident" means is helpful and should be incorporated into the
actual manuscript text, which currently is still confusing for readers
used to other meanings of the word: > "coincident" refers to the
proper analysis (the main search), when data from different detectors
are not time-shifted. It opposed to "background analysis".

A: we have added the sentence "The  coincident  search  is  the  proper  analysis  during which  true  GW  signals  are  searched  in  the  data."

L659ff: The\textbf{} answer given by the authors about using medians vs means
also seemed quite enlightening to me and I would encourage to include
a brief summary of it in the paper text.

A: we have added the explanation in the paper text.

Fig. 4 caption: "green are" -> "green curve"

A: mistake fixed

L789 and L851: Even with the replies by the authors, I still do not
understand what exactly the counting of "more triggers" in these two
sentences refer to. The discussed plot shows FAR as a function of
detection statistic, and the number of triggers must be a variable
along this curve. So at what FAR (or equivalently, pLambda) level are
those "more triggers" counted?

A: the total number of triggers is indeed no immediately visible on the FAR curves. The FAR curve for real data is above the curve for Gaussian noise, meaning that for a given value of pLambda, the FAR is higher with real data - to say it in another way, the number of noise trigger with a statistic higher than this value of pLambda is higher than with Gaussian noise.

We have tried to clarify this point l 855-856.
